Input Dropout for Spatially Aligned Modalities

Computer vision datasets containing multiple modalities such as color, depth, and thermal properties are now commonly accessible and useful for solving a wide array of challenging tasks. However, deploying multi-sensor heads is not possible in many scenarios. As such many practical solutions tend to be based on simpler sensors, mostly for cost, simplicity and robustness considerations. In this work, we propose a training methodology to take advantage of these additional modalities available in datasets, even if they are not available at test time. By assuming that the modalities have a strong spatial correlation, we propose Input Dropout, a simple technique that consists in stochastic hiding of one or many input modalities at training time, while using only the canonical (e.g. RGB) modalities at test time. We demonstrate that Input Dropout trivially combines with existing deep convolutional architectures, and improves their performance on a wide range of computer vision tasks such as dehazing, 6-DOF object tracking, pedestrian detection and object classification.

==> related_icip.tex <==
\subsection{Related work}

Using features from multiple modalities have been widely explored in the machine learning community. Various studies provides solutions to the questions such as which modalities are useful~\cite{wu2004optimal} and how should the modality be mixed into the same space~\cite{gunes2005affect, hu2015jointly, mees2016choosing, wagner2016multispectral} in order to distill useful information for a given task. Fusing the features often have the perverse side effect of making the network dependent on the extra modalities. 

% Privileged information
% Training a machine learning model with information that is not available at test time was dubbed ``training with privileged information'', and introduced by Vapnik et al.~\cite{vapnik2009new} as a new learning paradigm. It was demonstrated that using an additional source of information at training can improve the convergence rate~\cite{NIPS2010_3960} and multiple implementation of SVM~\cite{cortes1995support} support the theory~\cite{vapnik2015learning, xu2016simple, farquhar2006two}. Recently, this paradigm was transposed to deep learning~\cite{garcia2018learning, garcia2018modality,hoffman2016learning,neverova2016moddrop}. A method dubbed modality hallucination~\cite{hoffman2016learning} and its variants~\cite{garcia2018learning, garcia2018modality} proposes to train networks on different modalities independently and shows that by changing the input modality of one of the network while forcing the latent space to keep its former structure improves convergence. Nevertheless, these methods are quite complex to implement, require multiple training steps, and must be adapted differently to each problem. 

\textbf{Neverova et al.~\cite{neverova2016moddrop} proposed to train a neural network on multiple modalities while applying a \emph{modality dropout} to make the network invariant to missing modalities.} In this paper, we propose to explore this idea and extend the experimentations on various datasets~\cite{xiao2013sun3d, garon2018framework,hwang2015multispectral, Silberman:ECCV12, sakaridis2018semantic}. \textbf{However, there are major differences, which will be presented in section 3, between the technique we propose in this paper and the one of \cite{neverova2016moddrop}.} 

% With the rise of data hungry machine learning methods such as deep neural networks, various datasets containing multiple modalities have been collected~\cite{xiao2013sun3d, garon2018framework,hwang2015multispectral, Silberman:ECCV12, sakaridis2018semantic} in order to solve different problems with the highest quality data available. Unfortunately, while datasets may contain extra modalities, it is more difficult to capture them in practical applications (e.g. at test time). For example, in 3D object tracking, methods take advantage of depth information to attain robust results~\cite{joseph2015versatile,garon2017deep,garon2018framework,krull2015learning}. However, depth cameras are costly and less power-efficient than passive RGB cameras, therefore designing practical methods that depend on depth is less practical. Thus, recent 3D tracking methods have shifted to RGB-only algorithms~\cite{tjaden2017real, li2018deepim, manhardt2018deep}. In other tasks such as dehazing, state of the art methods uses only RGB information for training~\cite{Li_2018_CVPR,yang2018towards}. With depth being highly correlated with haze, we show that datasets with depth such as NYU V2~\cite{Silberman:ECCV12} and Cityscape~\cite{sakaridis2018semantic} can be exploited to improve neural networks convergence.


